Secretary Problems with Non-Uniform Arrival Order

For many online problems, it is known that the uniform arrival order enables the design of algorithms with much better performance guarantees than under worst-case. The quintessential example is the secretary problem. If the sequence of elements is presented in uniformly random order there is an algorithm that picks the maximum value with probability 1/e, whereas no non-trivial performance guarantee is possible if the elements arrive in worst-case order. This work initiates an investigation into relaxations of the random-ordering hypothesis in online algorithms, by focusing on the secretary problems. We present two sets of properties of distributions over permutations as sufficient conditions, called the block-independence property and uniform-induced-ordering property. We show these two are asymptotically equivalent by borrowing some techniques from the approximation theory. Moreover, we show they both imply the existence of secretary algorithms with constant probability of correct selection, approaching the optimal constant 1/e in the limit. We substantiate our idea by providing several constructions of distributions that satisfy block-independence. We also show that {\Theta}(log log n) is the minimum entropy of any permutation distribution that permits constant probability of correct selection in the secretary problem with n elements. While our block-independence condition is sufficient for constant probability of correct selection, it is not necessary; however, we present complexity-theoretic evidence that no simple necessary and sufficient criterion exists. Finally, we explore the extent to which the performance guarantees of other algorithms are preserved when one relaxes the uniform random ordering assumption, obtaining a positive result for Kleinberg's multiple-choice secretary algorithm and a negative result for the weighted bipartite matching algorithm of Korula and Pal.

==> prelims.tex <==

%% \section{Model}
%% (question here: our main model is that there are two things that happen in parallel to generate the input sequence. an adversary assigns values to an abstract set of items, and independently nature --- or the algorithm, in a free order model --- samples the order in which those items appear in the input seq.)

%% (in a different model there is no adversary. there are items numbered 1,...,n in decreasing order of value, and nature puts them in a random order.)

%% (all of our positive results pertain to both models, obviously.)

%% (our negative results also pertain to both models, in some sense, i.e. for every negative result in the paper there are two ways of stating the result depending on which model; the proof is basically the same in most cases, but there are some differences e.g. the circuit complexity lower bound is much, much harder in the model with the adversary.)

\section{Preliminaries}
\label{sec:prelims}

We consider problems in which an algorithm
selects one or more element from a set $\items$ of $n$ items.
Items are presented sequentially, and
an algorithm may only select items at the 
time when they are presented.

In the {\em secretary problem} the items are 
totally ordered by value, and the algorithm is allowed
to select only one element of the input sequence,
with the goal of selecting the item of maximum value.
Algorithms for the secretary problem 
are assumed to be comparison-based\footnote{This 
assumption of comparison-based algorithms
is standard in the literature on secretary problems.
\citet{Samuels} proved that when the input order is 
uniformly random, it is impossible to achieve
probability of correct selection $1/\e + \eps$ for
any constant $\eps>0$, even if the algorithm is allowed
to observe the values.},
meaning their decision whether to 
select the item presented at time $t$
must be based only on the relative ordering
(by value) of the first $t$ elements that arrived.%
Algorithms are evaluated according to their
{\em probability of correct selection}, \ie
the probability of selecting the item of 
maximum value. 

To fix notation for secretary problems, it will be
convenient to assume that the set $\items$ of items
is $[n] = \{1,\ldots,n\}$. The order in which items
are presented is then represented by a permutation
$\natperm$ of $[n]$, where $\natperm(i)$ denotes the
position of item $i$ in the input sequence. Similarly,
the ordering of items by value can be represented by
a permutation $\advperm$ of $[n]$, where $\advperm(j)=i$
means that the $j^{\mathrm{th}}$ largest item is $i$.
Then, the input sequence observed by the algorithm
is completely described by the composition $\natperm \advperm$.
For any (possibly randomized) algorithm $\algo$, its
probability of correct selection when presented with
the input sequence described by $\natperm \advperm$ will
be denoted by $\pcs{\algo,\natperm \advperm}$. 

When stating performance guarantees for secretary problems
it will be useful to think of the problem as a game
between an algorithm designer and an adversary who chooses
the ordering of items by value, $\advperm$. When the 
algorithm designer selects randomized algorithm $\algo$,
the adversary samples the ordering $\advperm$ from a 
distribution $\advpd$ in $\dists{S_n}$ (the set of all
probability distributions on the permutation group $S_n$)
and nature samples the order in which items are presented
from distribution $\natpd \in \dists{S_n}$, the 
game's payoff is 
\[
\gval(\algo,\advpd) = \Ex{\pcs{\algo,\natperm \advperm} \growingmid
  (\natperm,\advperm) \from \natpd \times \advpd}.
\]
We denote the minimax value of the game simply by $\gval$.
If either $\algo$ or $\advpd$ is fixed, we denote by 
$\gval(\algo,\ast)$ or $\gval(\ast,\advpd)$ (respectively)
the payoff when the opponent plays a best response.
Thus, for example, the famous result of \citet{Lindley}
and \citet{Dynkin63} can be summarized by stating that 
when $\natpd$ is the uniform distribution,
$\gval = \frac{1}{\e} + o(1)$ as $n \to \infty$.

